Analyzing Linear Dynamical Systems: From Modeling to Coding and Learning

Encoding time-series with Linear Dynamical Systems (LDSs) leads to rich models with applications ranging from dynamical texture recognition to video segmentation to name a few. In this paper, we propose to represent LDSs with infinite-dimensional subspaces and derive an analytic solution to obtain stable LDSs. We then devise efficient algorithms to perform sparse coding and dictionary learning on the space of infinite-dimensional subspaces. In particular, two solutions are developed to sparsely encode an LDS. In the first method, we map the subspaces into a Reproducing Kernel Hilbert Space (RKHS) and achieve our goal through kernel sparse coding. As for the second solution, we propose to embed the infinite-dimensional subspaces into the space of symmetric matrices and formulate the sparse coding accordingly in the induced space. For dictionary learning, we encode time-series by introducing a novel concept, namely the two-fold LDSs. We then make use of the two-fold LDSs to derive an analytical form for updating atoms of an LDS dictionary, i.e., each atom is an LDS itself. Compared to several baselines and state-of-the-art methods, the proposed methods yield higher accuracies in various classification tasks including video classification and tactile recognition.

==> sec_proofs.tex <==
\section{Proofs}
\label{sec:proofs}

We present the proofs of Theorems \ref{Th:linear_combination}-\ref{Th:skew-column-U}. For better readability, we repeat the theorems before the proofs.
\setcounter{theorem}{0}
%\newtheorem{theorem}{Theorem}
\begin{theorem}\label{Th:linear_combination}
Suppose $\Mat{V}_1,\Mat{V}_2,\cdots,\Mat{V}_M\in \mathcal{S}(n,\infty)$, and  $y_1,y_2,\cdots,y_M\in \mathbb{R}$, we have
\begin{eqnarray}
\nonumber \parallel\sum_{i=1}^{M}y_i\Pi(\Mat{V}_i)\parallel_{F}^2 &=& \sum_{i,j=1}^{M}y_iy_j\parallel\Mat{V}_i^{\mathrm{T}}\Mat{V}_j\parallel_{F}^2,
\end{eqnarray}
\end{theorem}
%\nonumber  &=& \sum_{i,j=1}^{J}y_iy_j\parallel\Mat{V}_{ij}\parallel_{F}^2

\begin{proof}
We denote the $t$-order sub-matrix of the extended observability matrix $\Mat{O}_i$ as $\Mat{O}_i(t) = [\Mat{C}_{i}^{\mathrm{T}},(\Mat{C}_{i}\Mat{A}_{i})^{\mathrm{T}},\cdots,(\Mat{C}_{i}\Mat{A}_{i}^{t})]^{\mathrm{T}}$ by taking the first $t$ rows. We suppose that the Cholesky decomposition matrix for $\Mat{O}_i$ is $\Mat{L}_i$ and denote that $\Mat{V}_i(t)=\Mat{O}_i(t)\Mat{L}_i^{\mathrm{-T}}$. Then, we derive
\begin{eqnarray}\label{emnedding_proof}
\nonumber && \parallel\sum_{i=1}^{J}y_i\Pi(\Mat{V}_i)\parallel_{F}^2 \\
\nonumber
&& = \lim_{t\rightarrow\infty}\parallel\sum_{i=1}^{M}y_i\Mat{V}_i(t)\Mat{V}_i(t)^{\mathrm{T}}\parallel_{F}^2\\
\nonumber && =
\lim_{t\rightarrow\infty}\mathrm{Tr}\left(\sum_{i=1}^{M}y_i\Mat{V}_i(t)\Mat{V}_i(t)^{\mathrm{T}} \sum_{j=1}^{J}y_j\Mat{V}_j(t)\Mat{V}_j(t)^{\mathrm{T}}\right)\\
\nonumber  && = \lim_{t\rightarrow\infty}\sum_{i,j=1}^{M}y_iy_j\mathrm{Tr}\left(\Mat{V}_i(t)^{\mathrm{T}}\Mat{V}_j(t) \Mat{V}_j(t)^{\mathrm{T}}\Mat{V}_i(t)\right)\\
\nonumber  && = \sum_{i,j=1}^{M}y_iy_j\lim_{t\rightarrow\infty}\parallel\Mat{V}_i(t)^{\mathrm{T}}\Mat{V}_j(t)\parallel_F^2\\
\nonumber  && = \sum_{i,j=1}^{M}y_iy_j\lim_{t\rightarrow\infty}\parallel\Mat{L}_i^{-1}(\Mat{O}_i(t)^{\mathrm{T}} \Mat{O}_j(t))\Mat{L}_j^{\mathrm{-T}}\parallel_F^2\\
&& =
\sum_{i,j=1}^{M}y_iy_j\parallel\Mat{L}_i^{-1}\Mat{O}_{ij}\Mat{L}_j^{\mathrm{-T}}\parallel_F^2,
\end{eqnarray}
where the limitation value $\Mat{O}_{ij}=\lim_{t\rightarrow\infty}\Mat{O}_i(t)^{\mathrm{T}} \Mat{O}_j(t)=\Mat{O}_i^{\mathrm{T}}\Mat{O}_j$ exists and is computed by solving the Lyapunov equation similar to Eq. (\ref{Eq:Lyapunov1}).
\end{proof}

The Frobenius distance $\parallel\Pi(\Mat{V}_1)-\Pi(\Mat{V}_2)\parallel_{F}^2$ in Corollary \ref{metric} is devised by setting $y_1=1$ and $y_2=-1$ in Theorem \ref{Th:linear_combination}.

As demonstrated in \cite{harandi2013dictionary}, the embedding $\Pi(\Mat{V})$ from the finite Grassmannian $\mathcal{G}(n,d)$ to the space of the symmetric matrices is proven to be diffeomorphism  (a one-to-one, continuous, and
differentiable mapping with a continuous and differentiable inverse); The  Frobenius distance between the two points $\Mat{V}_1$ and $\Mat{V}_2$  in the embedding space can be rewritten as
\begin{eqnarray}\label{Eq:Frobenius distance}
\parallel\Mat{V}_1\Mat{V}_1^{\mathrm{T}}-\Mat{V}_2\Mat{V}_2^{\mathrm{T}}\parallel_{F}^2=2\sum_{k=1}^{n}\sin^2\alpha_k,
\end{eqnarray}
where $\alpha_k$ is the $k$-th principal angle of the subspaces between $\Mat{V}_1$ and $\Mat{V}_2$.

We denote the space of the finite observability subspaces as $\mathcal{S}(n,L)$ by taking the first $L$ rows from the extended observability matrix. Clearly, $\mathcal{S}(n,L)$ is a closed subset of $\mathcal{G}(n,L)$. Hence $\mathcal{S}(n,L)$ maintain the relation in Eq. (\ref{Eq:Frobenius distance}); and the embedding $\Pi(\Mat{V})$ from $\mathcal{S}(n,L)$  to the space of the symmetric matrices is diffeomorphism. For our case, $\mathcal{S}(n,\infty)=\lim_{L\rightarrow\infty}\mathcal{S}(n,L)$. Theorem (\ref{Th:linear_combination}) proves the Frobenius distance defined in the embedding $\Pi(\mathcal{S}(n,\infty))$ to be convergent. Thus, we can obtain the relation between the Frobenius distance and the subspace angles in Corollary \ref{metric}, and prove that the embedding $\Pi(\mathcal{S}(n,\infty))$ is diffeomorphism in Corollary \ref{diffeomorphism}, by extending the conclusions of $\mathcal{S}(n,L)$ with $L$ approaching to the infinity.


\begin{lemma}\label{canonical-representaion}
For a symmetric or skew-symmetric transition matrix $\Mat{A}$, the system tuple $(\Mat{A},\Mat{C})\in \mathbb{R}^{n \times n}\times\mathbb{R}^{m \times n}$ has the canonical form $(\Mat{\Lambda},\Mat{U})\in \mathbb{R}^{n}\times\mathbb{R}^{m \times n}$, where $\Mat{\Lambda}$ is diagonal and $\Mat{U}$ is unitary, \ie $\Mat{U}^\ast\Mat{U}= \mathbf{I}$. Moreover, both $\Mat{\Lambda}$ and $\Mat{U}$ are real if $\Mat{A}$ is symmetric and complex if $\Mat{A}$ is skew-symmetric; for the skew-symmetric $\Mat{A}$, $(\Mat{\Lambda},\Mat{U})$ is parameterized by a real matrix-pair $(\Mat{\Theta},\Mat{Q})\in \mathbb{R}^{n}\times\mathbb{R}^{m \times n}$ where $\Mat{\Theta}$ is diagonal and $\Mat{Q}$ is orthogonal.
\end{lemma}
\begin{proof}
\TODO{can we have just one citation, preferable a book for the symm/skew-symm decomposition?}

A symmetric or skew-symmetric matrix $\Mat{A}$ can be decomposed as $\Mat{A}=\Mat{U}\Mat{\Lambda}\Mat{U}^\ast$~\cite{Normal}.
Here $\Mat{U}$ is a unitary matrix and $\Mat{\Lambda}$ is a diagonal matrix storing the eigenvalues of $\Mat{A}$ .
For a symmetric matrix, both $\Mat{U}$ and  $\Mat{\Lambda}$ are real. For an skew-symmetric matrix,
the diagonal elements of $\Mat{\Lambda}$ and the columns of $\Mat{U}$ are
\begin{eqnarray}\label{Eq:skew-decomposition-lambda}
[\Mat{\Lambda}]_{2k-1} = [\Mat{\Theta}]_k \cdot 1i;~~~[\Mat{\Lambda}]_{2k} = -[\Mat{\Theta}]_k \cdot 1i,
\end{eqnarray}
and
\begin{eqnarray}\label{Eq:skew-decomposition-U}
\left\{
\begin{array}{lll}
 &\left[\Mat{U}\right]_{2k-1} & = \frac{1}{\sqrt{2}}[\Mat{Q}]_{2k-1} + \frac{1i}{\sqrt{2}}[\Mat{Q}]_{2k}, \\
 &\left[\Mat{U}\right]_{2k}   & = \frac{1}{\sqrt{2}}[\Mat{Q}]_{2k-1} - \frac{1i}{\sqrt{2}}[\Mat{Q}]_{2k},
\end{array}
\right.
\end{eqnarray}
for $k=1,2,\cdots,\frac{n}{2}$ if $n$ is even\footnote{When $n$ is odd, the first $n-1$ columns of $\Mat{\Lambda}_{s}$ are the same as Eq. (\ref{Eq:skew-decomposition-lambda}); the $n$-th element of $\Mat{\Lambda}$ is $0$. Our developments can be applied verbatim to this case as well.}, where $\Mat{\Theta}\in\mathbb{R}^{\frac{n}{2}\times\frac{n}{2}}$ is a real diagonal matrix and $\Mat{Q}\in\mathbb{R}^{m\times n}$ is a real orthogonal matrix. Thus $(\Mat{\Lambda},\Mat{U})$ can be parameterized by $(\Mat{\Theta},\Mat{Q})$ which is of real value.
\end{proof}




\begin{theorem}\label{Th:DL}
If we encode the data sequences with the two-fold LDS defined in Eq. (\ref{Eq:two-fold}) and constrain the transition matrices of the dictionary atoms to be either symmetric or skew-symmetric, then the sup-problem in Eq. (\ref{Eq:subproblem}) is equivalent to
\begin{eqnarray}\label{Eq:DL2}
\begin{aligned}
 & \min_{\Mat{U}_{r}^{(d)}, \Mat{\Lambda}_{r}^{(d)}}  &  &\sum_{k=1}^{n}[\Mat{U}_{r}^{(d)}]_k^*\Mat{S}_{r,k}[\Mat{U}_{r}^{(d)}]_k\\
 & ~~~\mathrm{s.t. }                       &  & (\Mat{U}_{r}^{(d)})^*\Mat{U}_{r}^{(d)}=\Mat{I}_n;\\
 &&& -1<\lambda_{r,k}^{(d)}<1,~1\leq k\leq n.
\end{aligned}
\end{eqnarray}
\vskip -0.1in \noindent
Here, $\Mat{S}_{r,k} = \sum_{i=1}^{I}\Mat{Z}_{r,i}(\sum_{j=1,j\neq r}^{2J}\Mat{Z}_{j,i}\Mat{F}_{r,j,k} -\Mat{F}_{r,i,k}^{(sym)}-\Mat{F}_{r,i,k}^{(skew)})$; $\Mat{F}_{r,j,k}$, $\Mat{F}_{r,i,k}^{(sym)}$ and $\Mat{F}_{r,i,k}^{(skew)}$ are defined in Eq. (\ref{Eq:krj}-\ref{Eq:kri}). The number of the dictionary atoms is $2J$ basically because both the symmetric and skew-symmetric dictionary are of size $J$.
\end{theorem}

We first derive several preliminary results prior to the proof of this theorem.

Section \ref{Sec:DL_two-fold} devises that both the data and dictionary tuple have the compact representation $(\Mat{\Lambda},\Mat{U})$ where $\Mat{\Lambda}$ is diagonal and $\Mat{U}$ is unitary. We denote the corresponded extended observability matrix of $(\Mat{\Lambda},\Mat{U})$ is $\Mat{O}$. Computing the self-inner-product obtains
\begin{eqnarray}
\nonumber && \Mat{O}^{\mathrm{T}}\Mat{O} \\
\nonumber && = \sum_{t=0}^{\infty}(\Mat{\Lambda}^{*})^t\Mat{\Lambda}^t, \\
&& = \mathrm{diag}([\frac{1}{1-|\lambda_{1}|^2}, \frac{1}{1-|\lambda_{2}|^2},\cdots,\frac{1}{1-|\lambda_{n}|^2}]),
\end{eqnarray}
where $\lambda_{1},\lambda_{2},\cdots,\lambda_{n}$ are the diagonal elements of $\Mat{\Lambda}$. In Section \ref{Sec:O}, we show for common extended observability matrix that the inner-product is computed via Lyapunov equation, where the explicit form of the inner-product is intractable to obtain. Due to the benefit of the two-fold LDS modeling, we here can explicitly devise the inner-product, which is paramount for the later calculations of the Cholesky decomposition matrix and the kernel functions in Eq (\ref{Eq:krj}-\ref{Eq:kri}).

Considering $\Mat{L}\Mat{L}^\mathrm{T}=\mathrm{Chol}(\Mat{O}^{\mathrm{T}}\Mat{O})$, the Cholesky decomposition matrix is equal to
$$\Mat{L} = \mathrm{diag}([\frac{1}{(1-|\lambda_{1}|^2)^{1/2}}, \frac{1}{(1-|\lambda_{2}|^2)^{1/2}},\cdots,\frac{1}{(1-|\lambda_{n}|^2)^{1/2}}]).
$$

For simplicity, we respectively denote the compact system tuples, the Cholesky decomposition matrix and the extended observability subspace of dictionary atom $\Mat{D}_j$ as $(\Mat{\Lambda}_j,\Mat{U}_j)$, $\Mat{L}_j$ and $\Mat{V}_j$, by dropping out the superscript $^{(d)}$. Thus, the kernel value between dictionary atoms in Eq. (\ref{Eq:gamma}) is computed as
\begin{eqnarray} \label{Eq:krj_derivation}
\nonumber
&& K(\Mat{D}_r,\Mat{D}_j) \\
\nonumber
&=& \parallel\Mat{V}_r^{\mathrm{T}}\Mat{V}_j\parallel_F^2 \\
\nonumber
&=&
\parallel\Mat{L}_r^{-1}\sum_{t=0}^{\infty}(\Mat{\Lambda}_r^{*})^t\Mat{U}_r^{*} \Mat{U}_j\Mat{\Lambda}_j^t\Mat{L}_j^{-\mathrm{T}}\parallel_{F}^2 \\
\nonumber
&=&
\mathrm{Tr}\left( \Mat{L}_r^{-1}\left(\sum_{t_1=0}^{\infty}(\Mat{\Lambda}_r^{*})^{t_1}\Mat{U}_r^{*} \Mat{U}_j\Mat{\Lambda}_j^{t_1}\right)\Mat{L}_j^{-\mathrm{T}} \Mat{L}_j^{-1}\left(\sum_{t_2=0}^{\infty}(\Mat{\Lambda}_j^{*})^{t_2}\Mat{U}_j^{*} \Mat{U}_r\Mat{\Lambda}_r^{t_2}\right)\Mat{L}_r^{-\mathrm{T}}
\right)\\
\nonumber
&=&
\sum_{t_1=0}^{\infty}\sum_{t_2=0}^{\infty}\mathrm{Tr}\left(
\Mat{L}_r^{-1}(\Mat{\Lambda}_r^{*})^{t_1})\Mat{U}_r^{*} \Mat{U}_j\Mat{\Lambda}_j^{t_1}(\Mat{L}_j^{-\mathrm{T}} \Mat{L}_j^{-1})(\Mat{\Lambda}_j^{*})^{t_2}\Mat{U}_j^{*} \Mat{U}_r((\Mat{\Lambda}_r)^{t_2}\Mat{L}_r^{-\mathrm{T}})
\right)\\
\nonumber
&=&
\sum_{t_1=0}^{\infty}\sum_{t_2=0}^{\infty}\sum_{k=1}^n
(1-|\lambda_{r,k}|^2)^{\frac{1}{2}}(\lambda_{r,k}^{*})^{t_1}[\Mat{\hat{U}}_r]_k^{*} \Mat{U}_j\Mat{\Lambda}_j^{t_1}(\Mat{L}_j^{-\mathrm{T}} \Mat{L}_j^{-1})(\Mat{\Lambda}_j^{*})^{t_2}(\Mat{U}_j)^{*} [\Mat{U}_r]_k\lambda_{r,k}^{t_2}(1-|\lambda_{r,k}|^2)^{\frac{1}{2}}\\
\nonumber
&=&
\sum_{t_1=0}^{\infty}\sum_{t_2=0}^{\infty}\sum_{k=1}^n
[\Mat{U}_r]_k^{*} \Mat{U}_j((\lambda_{r,k}^{*})^{t_1}\Mat{\Lambda}_j^{t_1})
((1-|\lambda_{r,k}|^2)\Mat{L}_j^{-\mathrm{T}}\Mat{L}_j^{-1}) (\lambda_{r,k}^{t_2}(\Mat{\Lambda}_j^{*})^{t_2})
(\Mat{U}_j)^{*} [\Mat{U}_r]_k\\
\nonumber
&=&
\sum_{k=1}^n
[\Mat{U}_r]_k^{*} \Mat{U}_j\left(\sum_{t_1=0}^{\infty}(\lambda_{r,k}^{*})^{t_1}\Mat{\Lambda}_j^{t_1}\right)
((1-|\lambda_{r,k}|^2)\Mat{L}_j^{-\mathrm{T}} \Mat{L}_j^{-1}) \left(\sum_{t_2=0}^{\infty}\lambda_{r,k}^{t_2}(\Mat{\Lambda}_j^{*})^{t_2}\right)
(\Mat{U}_j)^{*} [\Mat{U}_r]_k\\
&=&
\sum_{k=1}^n
[\Mat{U}_r]_k^{*}\Mat{F}_{r,j,k}[\Mat{U}_r]_k,
\end{eqnarray}
where the matrix $\Mat{F}_{r,j,k}=\Mat{U}_j\Mat{E}_{r,j,k}\Mat{U}_j^{*} $; and $\Mat{E}_{r,j,k}$ is a diagonal matrix with the value given by
$
\Mat{E}_{r,j,k} = \mathrm{diag}( [\frac{(1-|\lambda_{r,k}|^2)(1-|\lambda_{j,1}|^2)}{|1-\lambda_{r,k}\lambda_{j,1}^*|^2} ,\cdots, \frac{(1-|\lambda_{r,k}|^2)(1-|\lambda_{j,n}|^2)}{|1-\lambda_{r,k}\lambda_{j,n}^*|^2}] ).
$

So far, we obtain the result in Eq. (\ref{Eq:krj}). For the kernel function across the dictionary atom and data sequence, \emph{i.e.} $k(\Mat{D}_r,\Mat{X}_i)$ in Eq. (\ref{Eq:kri}) can be derived in the similar way as Eq (\ref{Eq:krj_derivation}).

By substituting the devised kernel values into Eq. (\ref{Eq:gamma}), we can deduce the objective function in Eq. (\ref{Eq:DL2}), thereby completing the proof of Theorem \ref{Th:DL}.


%\begin{remark}
%If we enforce all the transition matrices of the dictionary atoms and the input data to be the same multiple of identity, \emph{i.e.} $\Mat{\Sigma}_j = \Mat{A}_{x,i}=\sigma\Mat{I},j=1,\cdots,J,i=1,\cdots,I$, then the matrix $\Mat{S}(r,k)$ in Pro. (\ref{dictionary learning1}) becomes
%\begin{eqnarray}
%\Mat{S}(r) &=&  \sum_{i=1}^{I}\sum_{j=1,j\neq r}^{J}[\Mat{Z}_i]_r[\Mat{Z}_i]_j\Mat{U'}_j\Mat{U'}_j^{\mathrm{T}} -2\sum_{i=1}^{I}[\Mat{Z}_i]_r\Mat{C}_{x,i}\Mat{C}_{x,i}^{\mathrm{T}},
%\end{eqnarray}
%which all the transition matrices vanish. The columns of the optimal measurement matrix $\Mat{U'}_r$ for Pro. (\ref{dictionary learning1}) are the eigenvectors of $\Mat{S}(r)$ corresponding to its $n$ smallest eigenvalues.
%\end{remark}p

\begin{theorem}\label{Th:sym-column-U}
We denote $[\Mat{U}_{sym,r}^{(d)}]_{-k}\in \mathbb{R}^{m\times (n-1)}$ as the sub-matrix of $\Mat{U}_{sym,r}^{(d)}$ by removing the $k$-th column, i.e. $[\Mat{U}_{sym,r}^{(d)}]_{-k}=[[\Mat{U}_{sym,r}^{(d)}]_1,\cdots,[\Mat{U}_{sym,r}^{(d)}]_{k-1},[\Mat{U}_{sym,r}^{(d)}]_{k+1},\cdots,[\Mat{U}_{sym,r}^{(d)}]_n]$, and define $\Mat{W}=[\Mat{w}_{1},\cdots,\Mat{w}_{m-n+1}]\in\mathbb{R}^{m\times (m-n+1)}$ as the orthogonal complement basis of $[\Mat{U}_{sym,r}^{(d)}]_{-k}$. If $\Mat{u}\in \mathbb{R}^{(m-n+1)\times 1}$ is the eigenvector of  $\Mat{W}^{\mathrm{T}}\Mat{S}_{r,k}\Mat{W}$ corresponding to the smallest eigenvalue, then $\Mat{W}\Mat{u}$ is the optimal solution of $[\Mat{U}_{sym,r}^{(d)}]_{-k}$ for Eq. (\ref{Eq:DL-sym-U}).
\end{theorem}

\begin{proof}
Since $[\Mat{U}_{sym,r}^{(d)}]_k^{\mathrm{T}}[\Mat{U}_{sym,r}^{(d)}]_o=0$ for all $1\leq o\leq n, o\neq k$, then $[\Mat{U}_{sym,r}^{(d)}]_k$ lies in the orthogonal complement of the space spanned by the columns of $[\Mat{U}_{sym,r}^{(d)}]_{-k}$. Thus, there exists a vector $\Mat{u}\in \mathbb{R}^{(m-n+1)\times 1}$ satisfying $[\Mat{U}_{sym,r}^{(d)}]_k=\Mat{W}\Mat{u}$ and $\Mat{u}^{\mathrm{T}}\Mat{u}=1$. The objective function in Eq. (\ref{Eq:DL-sym-U}) becomes $\Mat{u}^{\mathrm{T}}(\Mat{W}^{\mathrm{T}}\Mat{S}_{r,k}\Mat{W})\Mat{u}$. Obviously, the optimal $\Mat{u}$ for minimizing this function is the eigenvector of the matrix $\Mat{W}^{\mathrm{T}}\Mat{S}_{r,k}\Mat{W}$ corresponding to the smallest eigenvalue.
\end{proof}

\begin{theorem}\label{Th:skew-column-U}
We denote $[\Mat{Q}]_{-2}\in \mathbb{R}^{m\times (n-2)}$ as the sub-matrix of $\Mat{Q}$ by removing the $(2k-1)$-th and $2k$-th columns, i.e. $[\Mat{Q}]_{-2}=[[\Mat{Q}]_1,\cdots,[\Mat{Q}]_{2k-2},[\Mat{Q}]_{2k+1},\cdots,[\Mat{Q}]_n]$, and define $\Mat{W}=[\Mat{w}_{1},\cdots,\Mat{w}_{m-n+2}]\in\mathbb{R}^{m\times (m-n+2)}$ as the orthogonal complement basis of $[\Mat{Q}]_{-2}$. If $\Mat{u}_1, \Mat{u}_2\in \mathbb{R}^{(m-n+1)\times 1}$ are the eigenvectors of  $\Mat{W}^{\mathrm{T}}\Mat{S'}_{r,k}\Mat{W}$ corresponding to the smallest two  eigenvalue, then $\Mat{W}\Mat{u}_1$ and $\Mat{W}\Mat{u}_2$ are the respective optimal solutions of $[\Mat{Q}]_{2k-1}$ and $[\Mat{Q}]_{2k}$ for Eq. (\ref{Eq:DL-skew-U}).
\end{theorem}
\begin{proof}
The proof is similar to Theorem \ref{Th:sym-column-U}.
\end{proof}

\section{The properties of two-fold LDSs}
The advantageous properties of two-fold LDSs are described in Section \ref{Sec:DL_two-fold}. Here we provide more details.

We first prove that the solution of $\Mat{A}_{sym}=\frac{1}{2}(\Mat{A}+\Mat{A}^{\mathrm{T}})$, $\Mat{A}_{skew}=\frac{1}{2}(\Mat{A}-\Mat{A}^{\mathrm{T}})$, and $\Mat{C}_1=\Mat{C}_2=\Mat{C}$ has the same modeling accuracy as that of the original LDS defined in Eq. (\ref{Eq:ARMA}). For the subspace method proposed in [], the system tuple $(\Mat{A},\Mat{C})$ is learned by minimizing the observation error $\Mat{w}_t$ and state error $\Mat{v}_t$. It derives $\Mat{C},\Mat{X}=\arg\min\parallel\Mat{Y}-\Mat{C}\Mat{X}\parallel_F$; and $\Mat{A}=\arg\min\parallel\Mat{X}_1-\Mat{A}\Mat{X}_0\parallel_{F}^2 $. By setting
$$\Mat{C}_1=\Mat{C}_2=\Mat{C},$$
$$\Mat{X}^{(1)}=\Mat{X}^{(2)}=\frac{1}{2}\Mat{X},$$
$$\Mat{A}_{sym}=\frac{1}{2}(\Mat{A}+\Mat{A}^{\mathrm{T}}), \Mat{A}_{skew}=\frac{1}{2}(\Mat{A}-\Mat{A}^{\mathrm{T}}),$$
we have the following equations:
\begin{eqnarray}
\parallel\Mat{Y}-\Mat{C}_1\Mat{X}^{(1)}-\Mat{C}_2\Mat{X}^{(2)}\parallel_F &=& \parallel\Mat{Y}-\Mat{C}\Mat{X}\parallel_F,
\end{eqnarray}
and
\begin{eqnarray}
\nonumber
&&   \parallel\Mat{X}_1^{(1)}+ \Mat{X}_1^{(2)}-(\Mat{A}_{sym}\Mat{X}_0^{(1)}+\Mat{A}_{skew}\Mat{X}_0^{(2)})\parallel_{F}\\
&=& \parallel\Mat{X}_1-\Mat{A}\Mat{X}_0\parallel_{F}.
\end{eqnarray}
It means that the observation and state errors caused by the two-fold LDS modeling keep the same as those of the original LDS.

Then we present that both $\Mat{A}_1$ and $\Mat{A}_1$ are guaranteed to be stable if $\Mat{A}$ is stabilized via the SN method. Note that the SN stabilization devises that
\begin{eqnarray}
\parallel\Mat{A}\parallel_2=\sqrt{\mu_{max}(\Mat{A}^{\mathrm{T}}\Mat{A})}=\sigma_{max}(\Mat{A})<1,
\end{eqnarray}
where $\mu_{max}$ and $\sigma_{max}$ compute the maximized eigenvalue and singular-value, respectively. Thus,
\begin{eqnarray}
\parallel\Mat{A}_1\parallel_2=\parallel\frac{1}{2}(\Mat{A}+\Mat{A}^{\mathrm{T}})\parallel_2\leq \frac{1}{2}(\parallel\Mat{A}\parallel_2+\parallel\Mat{A}^{\mathrm{T}}\parallel_2)<1.
\end{eqnarray}
Similarly, we also have $\parallel\Mat{A}_2\parallel_2<1$.

